InternVL-U: Democratizing Unified Multimodal Models for Understanding, Reasoning, Generation and Editing

Unified multimodal models (UMMs) that integrate understanding, reasoning, generation, and editing face inherent trade-offs between maintaining strong semantic comprehension and acquiring powerful generation capabilities. In this report, we present InternVL-U, a lightweight 4B-parameter UMM that democratizes these capabilities within a unified framework. Guided by the principles of unified contextual modeling and modality-specific modular design with decoupled visual representations, InternVL-U integrates a state-of-the-art Multimodal Large Language Model (MLLM) with a specialized MMDiT-based visual generation head. To further bridge the gap between aesthetic generation and high-level intelligence, we construct a comprehensive data synthesis pipeline targeting high-semantic-density tasks, such as text rendering and scientific reasoning, under a reasoning-centric paradigm that leverages Chain-of-Thought (CoT) to better align abstract user intent with fine-grained visual generation details. Extensive experiments demonstrate that InternVL-U achieves a superior performance - efficiency balance. Despite using only 4B parameters, it consistently outperforms unified baseline models with over 3x larger scales such as BAGEL (14B) on various generation and editing tasks, while retaining strong multimodal understanding and reasoning capabilities.

==> preamble.tex <==
\definecolor{citecolor}{HTML}{0071BC}

\definecolor{oursgray}{gray}{0.93} 


% define new commands here
\newcommand{\modelname}{InternVL-U\xspace}

%%%%%%%%%%%%
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\RequirePackage{xspace}
\makeatletter

\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\textit{e.g}\onedot} 
\def\Eg{\textit{E.g}\onedot}
\def\ie{\textit{i.e}\onedot} 
\def\Ie{\textit{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}

\makeatother

%%%%%%%%%%%%

\newcommand{\yes}{\ding{51}}
\newcommand{\no}{\ding{55}}
\newcommand{\graybox}[1]{\colorbox{gray!15}{#1}}
\newcommand{\gbf}[1]{\green{\bf{\fn{(#1)}}}}
\newcommand{\rbf}[1]{\gray{\bf{\fn{(#1)}}}}
\newcommand{\lsp}{\ \ \ \ --\ ~}
\newcommand{\rsp}{\ \ --\ \ \ ~}

\usepackage{CJK}


\newcommand{\TODO}[1]{\begin{CJK}{UTF8}{gbsn}\textcolor{red}{[todo: #1]}\end{CJK}}

\newcommand{\prompt}[1]{\textcolor{black}{\footnotesize{\texttt{#1}}}}


% \definecolor{myblue}{HTML}{3859FF}
% \definecolor{myblue}{HTML}{DEF2FA}
\definecolor{myblue}{HTML}{d6f0ff}
% \definecolor{myblue}{HTML}{DBF5F0}
% \definecolor{myblue}{HTML}{C0DEFA}

\newcommand{\mytoprule}{
    \toprule
    \noalign{\vspace{-0.2mm}}
}

\newcommand{\mymidrule}{
    \noalign{\vspace{-0.8mm}}
    \midrule
    \noalign{\vspace{-1mm}}
}

\newcommand{\mybottomrule}{
    \noalign{\vspace{-0.6mm}}
    \bottomrule
}

\hyphenation{InternVL}

% table
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}

% \newcommand\blfootnote[1]{%
% \begingroup
% \renewcommand\thefootnote{}\footnote{#1}%
% \addtocounter{footnote}{-1}%
% \endgroup
% }

\definecolor{baselinecolor}{gray}{.9}
\definecolor{reduce-color}{RGB}{67,178,68}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\green}[1]{\textcolor[RGB]{96,177,87}{#1}}
\newcommand{\fn}[1]{\footnotesize{#1}}

% 定义自己的颜色
\definecolor{lightblue}{RGB}{152,182,234}
\definecolor{lightgreen}{RGB}{164,212,133}

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\definecolor{prompt}{rgb}{0.21,0.49,0.74}

\usepackage{array}

\usepackage[most]{tcolorbox}
\newcommand{\finding}[2]{
    % args:
    %   1: finding number
    %   2: finding text
    \vspace{-0.1cm}
    \begin{tcolorbox}[
        colback=white!90!gray,     % Soft ivory background
        colframe=teal!60!black,     % Deep navy frame color
        arc=5pt,                    % Less rounded corners for a modern look
        boxsep=5pt,                 % Inner margin between text and frame
        left=6pt,                  % Left margin within the box
        right=6pt,                 % Right margin within the box
        top=2pt,                    % Top margin within the box
        bottom=2pt,                 % Bottom margin within the box
        boxrule=0.8pt,              % Frame thickness
        drop shadow=gray!50!white,  % Subtle shadow effect for depth
        enhanced jigsaw             % Allows for the shadow effect and better arcs
    ]
    \vspace{-0.1cm}
        \paragraph{\textbf{\textit{Observation #1:}}}#2
    \vspace{-0.1cm}
    \end{tcolorbox}
    \vspace{-0.1cm}
}

\usepackage{textcomp}

% 自动开启和关闭中文环境
%%
\AtBeginDocument{\begin{CJK}{UTF8}{gbsn}\CJKtilde}
\AtEndDocument{\clearpage\end{CJK}}
%%

\definecolor{BoxBackground}{RGB}{240, 240, 240} % 浅灰色背景
\definecolor{BoxFrame}{RGB}{0, 0, 0} % 黑色边框
\definecolor{TitleBackground}{RGB}{0, 0, 0} % 标题背景颜色
\definecolor{TitleText}{RGB}{255, 255, 255} % 标题文字颜色
% 设置全局tcolorbox样式
\tcbset{
  academicbox/.style={
    boxsep=5pt,
    left=2pt,
    right=2pt,
    bottom=0.5pt,
    boxrule=0.5pt,
    colback=BoxBackground,
    colframe=BoxFrame,
    colbacktitle=TitleBackground,
    coltitle=TitleText,
    enhanced,
    attach boxed title to top left={yshift=-0.1in,xshift=0.1in},
    boxed title style={boxrule=0pt,colframe=white},
    title={#1},
  }
}
\newtcolorbox{AcademicBox}[1][]{academicbox=#1}
\newcommand{\nchar}{\textbackslash n}
